Magnetic and Structural Properties of 5d Osmate Double Perovskites Probed by Nuclear Magnetic Resonance

The combined effect of electronic correlation and strong spin-orbit-coupling(SOC) can give rise to a variety of exotic quantum phases. Double perovskites provide a simple structure to study the spin-orbit-lattice entangled states. In this thesis, focusing on the 5d osmate double perovskite system, we conduct a combination of work including theoretical model simulation, first-principle calculation, and nuclear magnetic resonance experiments to understand the fundamental physical properties of this material system.

==> dedication.tex <==
% Define your dedication statement here

\newcommand{\yourDedication}{A great dedication goes here.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Do not edit these lines unless you wish to customize
% the template
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{titlepage}
\begin{center}

\vspace*{\fill}
\yourDedication\\
\vspace*{\fill}

\end{center}
\end{titlepage}


==> epigraph.tex <==
% Define your quote and author for the epigraph here

\newcommand{\yourQuote}{A great quote to start the thesis}
\newcommand{\yourAuthor}{Wenyang Li}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Do not edit these lines unless you wish to customize
% the template
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{titlepage}
\begin{center}

\vspace*{\fill}
\yourQuote\\
\textit{\yourAuthor}
\vspace*{\fill}

\end{center}
\end{titlepage}


